Spinner: Scalable Graph Partitioning in the Cloud

Several organizations, like social networks, store and routinely analyze large graphs as part of their daily operation. Such graphs are typically distributed across multiple servers, and graph partitioning is critical for efficient graph management. Existing partitioning algorithms focus on finding graph partitions with good locality, but disregard the pragmatic challenges of integrating partitioning into large-scale graph management systems deployed on the cloud, such as dealing with the scale and dynamicity of the graph and the compute environment. In this paper, we propose Spinner, a scalable and adaptive graph partitioning algorithm based on label propagation designed on top of the Pregel model. Spinner scales to massive graphs, produces partitions with locality and balance comparable to the state-of-the-art and efficiently adapts the partitioning upon changes. We describe our algorithm and its implementation in the Pregel programming model that makes it possible to partition billion-vertex graphs. We evaluate Spinner with a variety of synthetic and real graphs and show that it can compute partitions with quality comparable to the state-of-the art. In fact, by using Spinner in conjunction with the Giraph graph processing engine, we speed up different applications by a factor of 2 relative to standard hash partitioning.

==> abstract.tex <==
%The ability to manage large graphs has become critical for the operation of
%several organizations. For instance, social networks store the underlying graph
%structure in graph databases and use graph processing systems for analytical
%purposes. Such systems typically distribute the graph across a datacenter,
%making graph partitioning an essential aspect for efficiency as it affects the
%communication overhead as well as load balancing.  

%Large-scale graph management systems, such as databases and graph analytics
%systems, are core components of several organizations, like a social network.
%Such systems typically distribute the underlying graph across a datacenter,
%making graph partitioning an essential aspect for efficiency as it affects the
%communication overhead as well as load balancing.  

%Partitioning the graph across the available resources plays a critical role
%(STRONGER) as it affects communication overhead as well as load balancing, and
%eventually the ability of the organization to analyze the graphs in a quick
%and efficient manner.

%Despite its importance, partitioning large graphs is a notoriously hard
%problem. People usually resort to simple heuristcs such as random partitioning.
%The problem becomes more difficult because graphs are dynamic.
Several organizations, like social networks, store and routinely analyze large
graphs as part of their daily operation. Such graphs are typically distributed
across multiple servers, and graph partitioning is critical for efficient graph
management. Existing partitioning algorithms focus on finding graph partitions
with good locality, but disregard the pragmatic challenges of integrating
partitioning into large-scale graph management systems deployed on the cloud,
such as dealing with the scale and dynamicity of the graph and the compute environment.
%Such architectures are characterized by the scale and  the dynamic
%nature of the graphs, and the dynamic nature of the underlying compute
%environment. Current approaches either do not scale well or are designed only
%for static graphs, making them impractical for incorporating them in a graph
%management system.  Existing partitioning algorithm focus on partitioning
%locality and are applicable only to static graphs.  Changes in the input graph
%or in the size of the underlying compute environment may force a
%re-partitioning, which can be an expensive task.

%In this paper, we aim at a solution that performs substantially better than the
%most practical solution currently used, hash partitioning, but is nearly as
%practical. 

In this paper, we propose \emph{\sys}, a scalable and adaptive graph
partitioning algorithm based on label propagation designed on top of the Pregel
model. \sys scales to massive graphs, produces partitions with locality and
balance comparable to the state-of-the-art and efficiently adapts the
partitioning upon changes.  We describe our fully decentralized algorithm and
its implementation in the Pregel programming model that makes it possible to
partition billion-vertex graphs. We evaluate \sys with a variety of synthetic
and real graphs and show that it can compute partitions with quality comparable
to the state-of-the art.  In fact, by using \sys in conjunction with the Giraph
graph processing engine, we speed up different applications by a factor of $2$
relative to standard hash partitioning.  

%Critically, unlike existing approaches used traditionally for partitioning, our
%approach can scale to billion-vertex graphs.

%At the same time, we extend the algorithm to efficiently adapt to changes
%either in the graph or the underlying compute environment.  

%We provide the details of our implementation and evaluate it using synthetic
%graphs but also a massive-scale real social network.


==> definition.tex <==
%Managing graphs and their computations in parallel and distributed environments,
%such as clouds, brings a number of daunting challenges \cite{}. First, most
%graph computations are data-driven and data-intensive, as they are characterized
%by an exploratory nature dictated by the graph structure, whereas only little
%computation is performed on each vertex or edge. Following this pattern, the
%computation of each vertex depends on that of its neighbours, creating and
%intricate network of data dependencies.

%In a parallel and distributed system, this network of dependencies translates
%into expensive communication and coordination operations between the computing
%nodes. Within this framework, proper partitioning of the graph is very important
%but even harder than for traditional parallel computation problems. In fact, the
%unstructured nature of graphs makes it difficult to anticipate the resulting
%structure of their computation, hindering an effective partitioning a-priori.
%This problem is worsened by their poor locality.

Before describing \sys, we outline how the characteristics of large-scale graph
management in the cloud drive our design decisions. We discuss the partitioning
quality objectives from an algorithmic point of view and, further, the features
that \sys must have to be  practical at scale in a cloud environment.

%At a high-level the objective of our partitioning algorithm is twofold: (i) to
%reduce communication overheads and (ii) to maintain a balanced workload.
%Operations on a distributed graph a cloud normally requires communication 

Although this discussion applies to graph management in general, here we use
graph analytics systems, like Pregel~\cite{Malewicz2010} and Graphlab
\cite{Low2012}, as examples. In a Pregel computation, vertices are spread across
machines, and a user-defined function is iteratively executed in parallel in a
series of so-called \emph{supersteps}. According to this mode, each vertex
shares state with the adjacent vertices through messages that may traverse the
network if the destination vertex resides on a different physical machine.  On
the other hand, Graphlab exports a shared-memory model, allowing vertices to
directly access the state of their neighbors, and employs a distributed locking
mechanism to enforce consistency guarantees.  In this case, graph dependencies
force the system to cross the network to acquire locks.  Due to these patterns,
graph computations are typically data-intensive and quickly become
network-bound, hindering application performance and system scalability.

%To ground the problem definition with a few examples, consider the Pregel
%large-scale graph processing framework \cite{Pregel}. 

In both these examples, communication occurs for the most part across the edges
of the graph. Therefore, our first objective is to find a partitioning that
minimizes the \emph{cut edges} of the underlying graph, that is, edges that
cross partitions and contribute to the network overhead.

At the same time, we require the partitions to be \emph{balanced}. It has been
shown in different contexts that workload skew can greatly degrade
performance~\cite{Gonzalez2012}.  In the case of such graph processing systems,
the load of a machine is proportional to the number of graph edges it holds.
Typically, the amount of computation a vertex performs depends on the number of
messages it receives, which is usually proportional to the number of edges the
vertex has. Thus, we require that partitions are balanced on the number of
edges.

Furthermore, unlike partitioning techniques used for community detection,
partitioning for the purpose of graph management requires that we control the
number of partitions. This is dictated by the available resources of the compute
environment, e.g. the number of machines.  Therefore, \sys must be able to
compute what is called \emph{k-way balanced partitioning}, where $k$ is the
number of partitions and it is an input parameter to the algorithm.

%In Section~\ref{sec:eval}, we will show that this can improve processing
%latency in the Giraph graph processing system by up to X\%.

%Communication can be minimized by an effective partitioning of the graph, as
%also shown by \cite{{Powergraph}}.  While the problem is orthogonal to
%different platforms, and our solution is general enough to be deployed to many
%of them, in this paper we focus on Pregel due to its popularity in both the
%industry and the academia.

%Since its introduction, Pregel has gained attention by both the industry and
% the academia. Thanks to its intuitive programming model, developers can write
% algorithms to process massive graphs across a large number of commodity
% machines, without the complexities of programming a parallel and distributed
% system. Pregel provides the developer with a simple vertex-centric API based
% on message-passing. A vertex has a unique identifier (ID) and a value, and it
% can exchange state with the other vertices through \emph{messages}.
%
%Inspired by the Bulk Synchronous Parallel (BSP) model, a Pregel computation
% comprises of a sequence of \emph{supersteps} divided by a global
% synchronisation barrier.  During each superstep a user-defined function $f$ is
% executed in parallel on each active vertex. At superstep $s$, for any given
% vertex $v$, $f$ is provided with the messages sent to the vertex during the
% previous superstep $s-1$. Based on the content of these messages, $f$ can
% modify the vertex value and send messages to the other vertices.
%%At the end of each superstep, a vertex can \emph{vote to halt} and enter the
% inactive state. An inactive vertex is not executed during the following
% superstep, unless it has received a message. The computation finishes when all
% the vertices have voted to halt and no message is in transit.
%
%In Pregel, the graph is split across a number of machines. A common way of
% splitting the graph across $N$ machines is to use \emph{hash partitioning}.
%%According to hash partitioning, given a hashing function $H(v)$, vertex $v$ is
% assigned to machine $n$ if $H(v)~ \emph{mod}~N = n$. The hashing function is
% commonly applied to the vertex ID. Hash partitioning is an effective strategy
% as it is lightweight and it produces balanced partitions, given a fairly
% uniformly distributed index set. However, the effect of using hash
% partitioning to split the graph across the machines is that vertices are
% assigned randomly.
%By assigning vertices randomly to each machine, the partitioning produces a
% large number of \emph{cut edges}. A cut edge is an edge whose endpoints are
% assigned to two different machines. In Pregel it is common for vertices to
% send messages over the edges, hence hash partitioning can create extensive
% network communication between machines to transmit messages. Depending on the
% network architecture, it can have substantial impact on runtime performance.

%Our goal is to design an algorithm that partitions a graph for the Pregel model
%to decrease the \emph{runtime} of graph computations. As such, the graph should
%be split \emph{k-way} across the number of computing nodes used to execute graph
%computations with the system. To minimise network communication, the algorithm
%should produce a low number of \emph{cut edges}. Usually, the load of each
%machine in a Pregel system is proportional to the number of edges assigned to
%that machine. Hence, the algorithm should encourage \emph{balanced} partitions
%on the number of \emph{edges}.

%As Pregel was designed to process Petabyte-scale graphs, the algorithm should be
%\emph{scalable} and a good fit to be computed by and practically integrated in a
%Pregel system itself. 

%Although with respect to the partitioning objects, \sys shares the same goal
%with other work, the cloud adds extra requirements.  XXX 

%As such, it should be based on a \emph{lightweight} heuristic that depends only
%on \emph{local} per-vertex information  without expensive global points of
%centralization.  
To be scalable, \sys must avoid expensive global points of centralization that
characterize other approaches like ~\cite{Karypis1995, Ugander2013}.  This
concept also underlies graph-parallel abstractions, like Pregel, that force
programmers to naturally express distributed algorithms.  \sys draws inspiration
from abstractions like Pregel and, in fact, we implement our algorithm in the
Pregel model.

The dynamic nature of both the graph and the compute environment calls for
specific design goals. Supporting efficient adaptation to changes requires that
\sys can compute partitions \emph{incrementally}. As opposed to discarding a
previous partitioning, \sys must be able to re-use it. Furthermore, \sys must be
able to handle different types of changes, such as additions and removals of
vertices or edges as well as changes to the number of partitions.  In the
following section, we describe in detail how \sys achieves these design goals.

